Metric Clustering and MST with Strong and Weak Distance Oracles

We study optimization problems in a metric space $(\mathcal{X},d)$ where we can compute distances in two ways: via a ''strong'' oracle that returns exact distances $d(x,y)$, and a ''weak'' oracle that returns distances $\tilde{d}(x,y)$ which may be arbitrarily corrupted with some probability. This model captures the increasingly common trade-off between employing both an expensive similarity model (e.g. a large-scale embedding model), and a less accurate but cheaper model. Hence, the goal is to make as few queries to the strong oracle as possible. We consider both so-called ''point queries'', where the strong oracle is queried on a set of points $S \subset \mathcal{X} $ and returns $d(x,y)$ for all $x,y \in S$, and ''edge queries'' where it is queried for individual distances $d(x,y)$. Our main contributions are optimal algorithms and lower bounds for clustering and Minimum Spanning Tree (MST) in this model. For $k$-centers, $k$-median, and $k$-means, we give constant factor approximation algorithms with only $\tilde{O}(k)$ strong oracle point queries, and prove that $\Omega(k)$ queries are required for any bounded approximation. For edge queries, our upper and lower bounds are both $\tilde{\Theta}(k^2)$. Surprisingly, for the MST problem we give a $O(\sqrt{\log n})$ approximation algorithm using no strong oracle queries at all, and a matching $\Omega(\sqrt{\log n})$ lower bound. We empirically evaluate our algorithms, and show that their quality is comparable to that of the baseline algorithms that are given all true distances, but while querying the strong oracle on only a small fraction ($<1\%$) of points.

==> MST_old_logn.tex <==
\section{Minimum Spanning Trees with only the Noisy Distance Oracle}
\label{sec:alg-mst}

Our results in \Cref{sec:alg-k-center}, \Cref{sec:alg-k-means}, and \Cref{sec:k-cluster-lb} have shown that there are strong separations between algorithms with and without the strong location oracle, and a sufficiently large number of strong oracle queries is necessary for $k$-clustering tasks. In light of this, a natural question is whether the strong oracle is necessary for all geometric problems. In this section, we answer this question in the negative: we show that for some other geometric problems, e.g., the minimum spanning trees (MST) problem, there exist good approximation algorithms with access \emph{only} to the noisy distance oracle.

We can first see intuitively why the lower bound in \Cref{sec:k-cluster-lb} does \emph{not} work against MST with large approximation factors. In the clustering task, the induced additive error becomes unbounded even if the algorithm fails to identify a single matched pair. However, for the MST problem, the optimal solution still has to pay the cost between different pairs; as such, even if the algorithm connects all the matches pairs with the ``wrong edge'', the induced cost is at most twice as large as the optimum. This observation gives us the hope to design algorithm with only the weak oracle by taking advantage of the lower bound of the optimal cost.

\subsection{Warm-up: The metric input of distances}
\label{subsec:mst-metric-input}
\chen{Writing note: if we end up not being able to solve the general version we need to change the narrative and primarily market the metric setting here}

\raj{Agreed, we should change how we sell this quite a bit. Specifically, one main motivation is where we have two embeddings -- one that is easier to compute, and one that is harder to compute. I can add this when I make a pass on the intro. }


\raj{The model should be formalized. Specifically, the marked entries are first chosen i.i.d.. Second, an adversary sees the marked entries, and can change them to any value so long as, after all changes are complete, the result is a metric.}
We first discuss the case when the distances by the corrupted noisy oracle are \emph{metric}, i.e., the adversary carefully perturb the distances such that for all triplet of vertices $(u,v,w)$, the triangle inequality and non-negativity still hold. We show that if we directly optimize the MST tree under $\dtilde$ (the corrupted distance oracle), the resulting tree is still a good approximation for the MST under $d$. More formally, we aim to prove the following lemma.
\raj{consider replacing $w$ with weight for something more explicit, since $w$ is also used to refer to a vertex}
\begin{lemma}
\label{lem:mst-alg-metric-case}
Let $\dtilde$ be the corrupted distance of $d$ that satisfy the metric property. Let $\Tstar_{d}$ and $\Tstar_{\dtilde}$ be the minimum spanning trees with distances from $d$ and $\dtilde$, respectively. Then, there is
\begin{align*}
\expect{w_{d}(\Tstar_{\dtilde})} \leq O(\log{n})\cdot w_{d}(\Tstar_{d}).
\end{align*}
\end{lemma}

It is straightforward to see that by \Cref{lem:mst-alg-metric-case}, we can simply run an MST algorithm with the corrupted distance metric $\dtilde$ and use the resulting tree to get an $O(1)$-approximation of the MST on $G$ without the precise location oracle. We will prove \Cref{lem:mst-alg-metric-case} in steps by a charging argument. To begin with, we first define a ball carving procedure similar to the proof in \Cref{sec:alg-k-center} and \Cref{sec:alg-k-means}. \raj{the nature of the ball carving here is actually quite different than in earlier sections, and is significantly more nuanced. We should make sure to emphasize this}

\chen{check and change these before the May 3 meeting}

\raj{The ball $\lball{\ell}{v}$ is with respect to the original metric $d$. Perhaps we should add $d$ or $\tilde{d}$ as a subscript to each ball to make it clear which metric the ball is defined with respect to. I did this for the ball in the lemma below.} 
\begin{definition}[$\ell$-heavy ball]
\label{def:level-ell-ball}
Fix any $\ell \geq 0$. 
For any vertex $v\in V$, we define the level-$\ell$ heavy radius at the vertex $v$ to be the smallest radius $r=r^{\ell}_{v}$ such that the metric ball $\ldball{d}{\ell}{v}{r}$ under the distance measure $d$, contains exactly $200 \cdot 2^{\ell}$ points in the dataset $V$. We define the level-$\ell$ heavy ball at $v$ to be the metric-ball $\ldball{d}{\ell}{v}{r^\ell_v}$ under the metric $d$. 
\end{definition}
\raj{above definition: need to clarify that you are defining the radius here. Also we are defining a ball in this definition, not a ball carving. I changed the def accordingly.}

\begin{lemma}[Probabilistic metric violation guarantee]
\label{lem:ball-distance-preserve}
Let $\dtilde$ be the corrupted distance of $d$ that satisfies the metric property. Fix any vertex $v\in V$ and let $\ball{v}{r_{v}}$ be the smallest ball that contains $200 \log(n)$ vertices centered at $v$. Then, with high probability, for any $x \in \ball{v}{r_{v}}$ and $y\in V$, the following inequalities hold:
\begin{align*}
& \dtilde(x,y) \leq d(x,y) + 2r_{v}; \\
& d(x,y) \leq \dtilde(x,y) + 2r_{v}.
\end{align*}
\end{lemma}
\begin{proof}

We use the high probability event of the preservation of distances and the properties of triangle inequalities to prove the lemma. For any fixed point $x$ in ball $\ball{v}{r_{v}}$ and a point $y\in V$, if we look at a point $z \in \ball{v}{r_{v}} \setminus \{x,y\}$, with probability $\frac{1}{9}$, the distances $\dtilde(y, z)$ and $\dtilde(x, z)$ are \emph{not} corrupted, i.e., $\dtilde(y,z)=d(y,z)$ and $\dtilde(x,z) = d(x, z)$. We define $S_{z}$ as the indicator random variable for the above event, and $S=\sum_{z\in \ball{v}{r_{v}} \setminus \{x,y\}} S_{z}$ as the total number of vertices in $\ball{v}{r_{v}}$ whose distances between $x$ and $y$ are preserved. By a simple calculation, there is $\expect{S}\geq 22 \log(n)$, and since the distances are corrupted \emph{independently}, we can apply Chernoff bound to the random variable $S$ and obtain
\begin{align*}
\Pr\paren{S \leq 1} &\leq \exp\paren{-2\cdot \frac{22^2 \log^2{n}}{200 \log(n)}}\\
&\leq \frac{1}{n^4}.
\end{align*}
Therefore, we can apply a union bound over ${n \choose 2}$ possible pairs of distances to obtain the guarantee on any ball and distance.

We now condition on this probabilistic guarantee to prove the lemma. Fix a point $x$ in $\ball{v}{r_{v}}$, a point $y\in V$, and a point $z$ such that $\dtilde(x,z)$ and $\dtilde(y,z)$ are preserved. For the first inequality, we have
\begin{align*}
\dtilde(x,y) &\leq \dtilde(x,z) + \dtilde(z,y) \tag{by the metric property of $\dtilde$}\\
&=d(x,z)+d(z,y) \tag{the distances are preserved}\\
&\leq r_{v} + d(x,z) + d(x,y) \tag{$d(x,z)\leq r_{v}$ and the metric property of $d$}\\
&\leq d(x,y) + 2 r_{v}.
\end{align*}
Similarly, for the second inequality, we have
\begin{align*}
d(x,y) &\leq d(x,z) + d(z,y) \tag{by the metric property of $d$}\\
&= d(x,z)+\dtilde(z,y) \tag{the distances are preserved}\\
&\leq r_{v} + \dtilde(x,z) + \dtilde(x,y) \tag{$d(x,z)\leq r_{v}$ and the metric property of $\dtilde$}\\
&= r_{v} + d(x,z) + \dtilde(x,y) \tag{the distance is preserved}\\
&\leq \dtilde(x,y) + 2r_{v},
\end{align*}
as desired.
\end{proof}
\chen{See if this argument extends to arbitrary-size balls -- need to be more careful about the union bound.}

We now use \Cref{lem:ball-distance-preserve} to prove the approximation guarantee for the MST. To begin with, we introduce the following thought process of ball carving:
\begin{algorithm}[!htbp]
\caption{\label{alg:thought-process-mst}A thought process of ball carving (\emph{not} an implemented algorithm)}
\KwData{Set of points $V$}
\textbf{Init:} $X=V$ \\

\While{$X\neq \emptyset$}{
    For each $v\in V$, let $\ball{v}{r_{v}}$ be the smallest ball with $200\log(n)$ points from $V$ centered at $v$ with radius $r_{v}$.\\ 
    Pick $v\in X$ such that $\ball{v}{r_{v}}$ attains the largest $r_{v}$ among the points of $V$.\\
    Let $S_{i}=\ball{v}{r_{v}}\cap X$, $x_{i}=v$, and $r_{i}=r_{v}$.\\
    Remove $S_{i}$ from $X$ and recurse.
}
\end{algorithm}

We emphasize that \Cref{alg:thought-process-mst} is \emph{not} implemented throughout and is only for analysis purposes. Crucially, \Cref{alg:thought-process-mst} gives us a way to lower bound the optimal cost of the MST.
\begin{claim}
\label{clm:mst-cost-lb-ball-carve}
Let $\Tstar_{d}$ be the minimum spanning tree of $G=(V,E)$ under distance $d$, there is
\begin{align*}
w_{d}(\Tstar_{d}) \geq \frac{1}{2}\cdot \sum_{i} r_{i},
\end{align*}
where $r_{i}$ are the radius of the balls from \Cref{alg:thought-process-mst}.
\end{claim}
\begin{proof}
We prove the claim by showing that the balls of radius $\ball{x_i}{\frac{r_i}{2}}$ are disjoint (where $x_{i}$ is the selected center of the ball of the $i$-th iteration). To see this, note that for a fix $i$, if $\ball{x_i}{\frac{r_i}{2}}$ contains a point of $z\in \ball{x_{j}}{r_j}$ for $j>i$, then the ball $\ball{x_i}{r_i}$ should have contained $x_{j}$ (since $r_{j}<r_{i}$), and $x_{j}$ should not have been selected during the ball carving process, which forms a contradiction. Similarly, if $\ball{x_i}{\frac{r_i}{2}}$ contains a point of $z\in \ball{x_{k}}{r_k}$ for $k<i$, then the ball $\ball{x_k}{r_k}$ should have contained $x_{i}$, and $x_{i}$ should not have been selected during the ball carving process. Finally, since the points in each $\ball{x_i}{\frac{r_i}{2}}$ are disjoint, the minimum spanning tree must enter and leave each ball, which pays at least $\frac{1}{2}\cdot \sum_{i} r_{i}$ in cost.
\end{proof}

Besides lower-bounding the MST cost as in \Cref{clm:mst-cost-lb-ball-carve}, we present two technical steps toward the proof of \Cref{lem:mst-alg-metric-case}.

\begin{lemma}
\label{lem:mst-corrupt-leq-true}
Let $\dtilde$ be the corrupted distance of $d$ that satisfy the metric property, and let $T$ be any spanning tree of $G=(V,E)$. With high probability, there is 
\begin{align*}
w_{\dtilde}(T)\leq w_{d}(T) + O(\log(n))\cdot w_{d}(\Tstar_{d}).
\end{align*}
\end{lemma}
\begin{proof}
We root the tree $T$ arbitrarily and define the charging scheme as follows.
\begin{tbox}
\underline{A Charging Scheme.} 
\begin{enumerate}
\item For each tree edge $(u,v)\in T$, suppose w.log. that $v$ is the child node. 
\item Find the center $x_{i}$ such that $v$ is included in $S_{i}$ of \Cref{alg:thought-process-mst}, distribute a charge of $d(u,v)+2\cdot r_i$ to $v$.
\end{enumerate}
\end{tbox}
We need to verify that the charge we distributed is enough for $\dtilde(u,v)$ -- this is the probabilistic part of this argument, where we condition on the high probability event of \Cref{lem:ball-distance-preserve}, and argue that $\dtilde(u,v)\leq d(u,v)+2\cdot r_i$. As such, the charging scheme is sufficient to accommodate the charges from each $\dtilde(u,v)$.

We now upper bound the total charge that can be distributed. Note that the total charge is at most 
\begin{align*}
\sum_{(u,v)\in T} d(u,v)+2\cdot r_i \leq \sum_{(u,v)\in T} d(u,v) + 2\cdot O(\log(n)) \sum_{i}r_i,
\end{align*}
where the latter part of the inequality comes from the fact each point (that brings a $r_{i}$ charge) can be charged at most once, and there are at most $O(\log(n))$ times of charges from each ball. Therefore, by using \Cref{clm:mst-cost-lb-ball-carve}, we have
\begin{align*}
w_{\dtilde}(T) &\leq w_{d}(T) + 4\cdot O(\log(n))\cdot w_{d}(\Tstar_{d}),
\end{align*}
as desired.
\end{proof}

We also bound the lemma in the `reverse' direction that upper bounds the weights on $d$ with the distances on $\dtilde$.

\begin{lemma}
\label{lem:mst-true-leq-corrupt}
Let $\dtilde$ be the corrupted distance of $d$ that satisfy the metric property, and let $T$ be any spanning tree of $G=(V,E)$. With high probability, there is 
\begin{align*}
w_{d}(T)\leq w_{\dtilde}(T) + O(\log(n))\cdot w_{d}(\Tstar_{d}).
\end{align*}
\end{lemma}
\begin{proof}
The proof follows the same idea as we used in \Cref{lem:mst-corrupt-leq-true} -- again, we root the tree $T$ arbitrarily and define the charging scheme as follows.
\begin{tbox}
\underline{A Charging Scheme.} 
\begin{enumerate}
\item For each tree edge $(u,v)\in T$, suppose w.log. that $v$ is the child node. 
\item Find the center $x_{i}$ such that $v$ is included in $S_{i}$ of \Cref{alg:thought-process-mst}, distribute a charge of $\dtilde(u,v)+2\cdot r_i$ to $v$.
\end{enumerate}
\end{tbox}
By conditioning on the high probability event of \Cref{lem:ball-distance-preserve} (second inequality), we can again argue that $d(u,v)\leq \dtilde(u,v)+2\cdot r_i$, and the charging scheme is sufficient to accommodate the charges from each $d(u,v)$. Furthermore, we can similarly upper-bound the total charge that can be distributed as
\begin{align*}
\sum_{(u,v)\in T} \dtilde(u,v)+2\cdot r_i &\leq \sum_{(u,v)\in T} \dtilde(u,v) + 2\cdot O(\log(n)) \sum_{i}r_i\\
&\leq \cdot w_{\dtilde}(T) + O(\log(n))\cdot w_{d}(\Tstar_{d}),
\end{align*}
as desired.
\end{proof}

\paragraph{Wrapping up the proof of \Cref{lem:mst-alg-metric-case}.} Let $\Tstar_{\dtilde}$ and $\Tstar_{d}$ be the MSTs obtained with respect to distance metric $\dtilde$ and $d$, respectively. We have
\begin{align*}
w_{d}(\Tstar_{\dtilde}) &\leq w_{\dtilde}(\Tstar_{\dtilde}) + O(\log(n))\cdot w_{d}(\Tstar_{d}) \tag{by \Cref{lem:mst-true-leq-corrupt}}\\
&\leq w_{\dtilde}(\Tstar_{d}) + O(\log(n))\cdot w_{d}(\Tstar_{d}) \tag{$\Tstar_{\dtilde}$ is the minimum spanning tree under $\dtilde$}\\
&\leq w_{d}(\Tstar_{d}) + O(\log(n))\cdot w_{d}(\Tstar_{d}) + O(\log(n))\cdot w_{d}(\Tstar_{d}) \tag{by \Cref{lem:mst-corrupt-leq-true}}\\
&=O(\log(n))\cdot w_{d}(\Tstar_{d}),
\end{align*}
as claimed by \Cref{lem:mst-alg-metric-case}.


==> warmup-alg.tex <==
\section{A Warm-up Algorithm}

\prat{Assumptions, algorithm and claim}

Let $\Cstar_{i}$ denote the ground truth set of points belonging to cluster $i$.
For now, we will work with the following assumptions

\begin{assumption}
\label{assmp:dreamland}
Let $\OPT$ be the optimal cost of $k$-center clustering, we assume the instance satisfies the following conditions:
\begin{enumerate}
\item $d(u,v) = \omega(1)\cdot \OPT$ for all $u \in \Cstar_{i}, \, v \in \Cstar_{j}, \, i\neq j$ .
\item For all $i\in [k]$, there is $\card{\OPTClus_{i}}\geq \eps \cdot n$ for some $\eps>0$.
\end{enumerate}
\end{assumption}



% \begin{assumption}

% \end{assumption}

% \begin{assumption}
% OPT and $d_i^*$ are known.
% \end{assumption}
\begin{theorem}
\label{thm:warmup-alg}
Conditioning on \Cref{assmp:dreamland}, there exists an algorithm that gives an $\frac{2}{1-o(1)}$ approximation for the k-center clustering problem under noisy oracle model.
\end{theorem}

The algorithm is as follows.

\begin{algorithm}[!htbp]
\caption{\label{alg:main}An algorithm conditioning on \Cref{assmp:dreamland}}
\KwData{Set of points $X$, number of centers $k$}
\KwData{Additional Oracle: the value of \OPT}
\textbf{Init:} $S_1 = \{u\}$ for some arbitrary $u \in X$ \\

\For{$i \gets 2,...,k$}{
    $|T_i| = 20 \log n/\eps^2$ points sampled u.a.r. from $X \setminus S_{i-1}$ \\
    % Query location oracle for $T_i \cup S_{i-1}$\\
    % Construct distances $d(u,v)$ for all vertex pairs $(u,v)\in T_i \cup S_{i-1}$ \\
    % \textbf{Distance test subroutine} -  \\
    % Assume we have $d_{i}^* \geq d(v, T_{i} \cup S_{i-1})$ for all $v \in X \setminus T_{i} \cup S_{i-1}$ \\
    Partition the points in $T_{i}\cup S_{i-1}$ as follows.\\
    \For{$j \in [i]$}{
        Query location oracle for each $w \in T_{i}$ and $s_{j}$, and obtain the actual distance $d(w, s_{j})$. \\
        If $d(w, s_{j}) \leq 2\cdot \OPT$, add $w$ to $\ESTClus_{j}$.\\
    }
    Estimate the distances between each $x \in X\setminus S_{i-1}\cup T_{i}$ and $S_{i-1}$ as follows.\\
    \For{$x \in X \setminus T_i \cup S_{i-1}$}{
        \For{$j \in [i]$}{
            $\dest_{j}(x, \ESTClus_{j})=\med{\{\dtilde(x,w)\mid w\in \ESTClus_{j}\}}$.
        }
        Let $\dest(x, S_{i-1})$ be the minimum distances among $\dest_{j}(x, \ESTClus_{j})$.
    }
    Pick the point $s$ such that $\dest(s,S_{i-1}) \geq \dest(x,S_{i-1})$ for all $x \in X\setminus S_{i-1}$. \\
    $S_{i} = \{s\} \cup S_{i-1}$.
    
}
\end{algorithm}

\pagebreak

\prat{Reintroduce notations here for simplicity?}

We now analyze \Cref{alg:main}. We start with bounding the number of distance and location queries.
\begin{lemma}
\label{lem:comp-assmp-alg}
\Cref{alg:main} makes at most $O\paren{nk\cdot \max\{k, \frac{\log(n)}{\eps}\}}$ distance queries and $O(\frac{k \log(n)}{\eps})$ location queries.
\end{lemma}
\begin{proof}
In each iteration, the distance and the location queries are made as follows. For each sampled point, we make distance queries between all points  in $X\setminus S_{i-1}\cup T_{i}$ and the points in each $\ESTClus_{j}$, $j\in [i]$, which is at most $O(\max\{k, \frac{\log(n)}{\eps}\})$ since $i\leq k$. As such, the number of distance queries we make in each iteration is at most $O(n\cdot \max\{k, \frac{\log(n)}{\eps}\})$. Furthermore, for each sampled point, we make one location query, and in the most extreme case where the points sampled in each iteration are disjoint, the number of location queries we ever make is at most $O(\frac{\log(n)}{\eps})$ in each iteration. Therefore, over the $k$ iterations, the number of distance and location queries are at most $O\paren{nk\cdot \max\{k, \frac{\log(n)}{\eps}\}}$ and $O(\frac{k \log(n)}{\eps})$, as claimed.
\end{proof}

Assuming $k<<n$ and $\eps$ be a constant, the number of distance and location queries become $O(n \log(n))$ and $O(\log(n))$ -- the exponential reduction of location queries is particularly useful when such queries are costly, which matches the motivations of our problem.

% \chen{The lemmas should go as follows.
% \begin{enumerate}
%     \item For the partition guarantee, we show two things: 1. Among the points in $\ESTClus_{j}$, there are at least $10\log(n)$ points from $\OPTClus_{j}$, and at most $5\log(n)$ points from $\OPTClus_{i}$ for any $i\neq j$.
%     \item For the distance guarantee, as long as the number of correct estimations are more than $\card{\{\dtilde(x,w)\mid w\in \ESTClus_{j}\}}/2$, we can return a \emph{correct} $d(x,w)$.
%     \item And since $\OPT = o(d(x,w))$, the estimation is a $(1+o(1))$ approximation to the shortest distance. 
%     \item As such, the point we pick at each iteration is an approximate furthest traversal -- show the approximation guarantee therein. 
% \end{enumerate}
% }


% \chen{The plan Nov/11 -- Nov/20:
% \begin{enumerate}
%     \item Write the algorithm and the proof. Check if $O(\frac{\log(n)}{\eps^2})$ sampling size of $T_i$ can be made $O(\frac{\log(n)}{\eps})$ instead.
%     \item If time, the immediate next step is to remove the assumption on the cluster size -- try to make it $O(\log(n))$.
% \end{enumerate}
% } 

% \begin{algorithm}
% \caption{Distance test subroutine}
% Query distance oracle $\dtilde(x,w)$ for $w \in T_{i} \cup S_{i-1}$ \\
%         % \;
%         For all $w \in T_i$, assign each point to closest center in $S_{i-1}$. \\
%         Let $C_{j}^{(i)}$ be set of points from $T_i$ assinged to center $j$ in $S_{i-1}$ \\
%         % $ST_\ell (x) = \{ w \in C_{j}^{(i)}  |  \dtilde(x,w) \geq \frac{1}{2} d_i^*  \}$ \\
%         % $ST_s (x) = \{ w \in C_{j}^{(i)}  |  \dtilde(x,w) < \frac{1}{2} d_i^*  \}$ \;
%         Set $d(x, S_{i-1}) =$ median of $\dtilde(x,v)$ for $v \in C_{j}^{(i)}$ \\
% \end{algorithm}

\prat{Absorb constants in $O()$?}

We now turn to the proof of the correctness of the algorithm. We begin by bounding the number of representative points for each cluster $(\widetilde{C}_j)$ at each stage of the algorithm.

\begin{lemma}
\label{lem:warmup-sample-size}
Sampling $T_i = 40 i \log{n}/\eps$ points u.a.r at each step $i = {2, 3, \dots k}$ of the algorithm gives us $\card{\widetilde{C}_j} \ge 20 \log{n}$ w.p. $1 - n^{-c_1}$ for all $1 \le j < i$.
\end{lemma}
\begin{proof}
At iteration $i$, we have $i-1$ centers and since we use location queries, we only need bound the number of points covered by these centers that are sampled. Since from assumption we have that size of each cluster is at least $\varepsilon n$, in expectation we have $40 \log n$ points for cluster $1, 2, \dots i-1$. Using Chernoff we obtain, 

\[\Pr[\card{\widetilde{C}_j} \leq 20 \log n ] \leq \exp{ \big( -5 \log n} \big) \]

Using union bound over all centers we obtain w.p. $1 - n^{-c_1}$ $\card{\widetilde{C}_j} \ge 20
\log n$ for all $j < i$.

\prat{We're good here as long as $k = O(1)$ i think.}

\end{proof}


%The following fact follows from the observation that using the `median trick', w.p. $1 - n^{-c_\delta}$ we have correct distance estimate to one of the point in $\widetilde{C}_j$, where $c_\delta$ is a constant that depends only on $\delta$, followed by triangle inequality. Recalling $\dest(x, \widetilde{C}_j)$ is the median distance to points in cluster $\widetilde{C}_j$


Next, we compare the distances estimated by algorithm to the true distances which are used by the farthest-traversal algorithm.

\begin{claim}
\label{claim:warmup-med-trick}
For any point $x \in X \setminus T_i \cup S_{i-1}$, iteration $i$ and the estimated distance to any center $s_j \in S_{i-1}$ $(\dest(x, s_j))$, we have depending on whether $x$ belongs to the ground truth cluster $C^*_j$

\begin{itemize}
    \item if $x \in C^*_j, \quad \dest(x, s_j) \le 4 \OPT$ .
    \item if $x \notin C^*_j, \quad \big(1 - o(1)\big) d(x, s_j) \leq \dest(x, s_j) \le  \big(1 + o(1)\big) d(x, s_j)$.
\end{itemize}



%$ | \dest(x,\widetilde{C}_j) - d(x, s_j) | \le 2 \OPT$. 
\end{claim}
\begin{proof}

From \cref{lem:warmup-sample-size}, we have $O(\log n)$ representative points for each cluster $j$, denoted by the set $\widetilde{C}_j$. For a particular point $x \in X \setminus T_i \cup S_{i-1}$, noisy query oracle gives us distance to all points in
$\widetilde{C}_j$. Letting $\dest(x, s_j)$ be the median of these distances, median trick gives us that w.p. $1 - n^{-c_2}$ the estimated distance is true distance to one of the points in $\widetilde{C}_j$. \chen{We need to be more precise here and explain it.}

Case 1: $x \notin C^*_j$

Since any two points belonging to the same cluster are at most $2\OPT$ distance apart and set $\widetilde{C}_j$ is formed using location queries that use true distance measures, using triangle inequality $\card{\dest(x, s_j) - d(x,s_j) } \le 2\OPT$.

From \cref{assmp:dreamland}, we have that $d(x,s_j) = \omega(1) \OPT$ since $x \notin C^*_j$. As a result,
\[\dest(x, s_j) \le d(x, s_j) + 2\OPT \le \Bigg(1 + \frac{2\OPT}{d(x, s_j)} \Bigg) d(x, s_j) \le \big(1 + o(1)\big) d(x,s_j)\]

Similar analysis gives us the inequality for the other side.


Case 2: $x \in C^*_j$

For $x \in C^*_j$, $d(x, s_j) \leq 2\OPT$ and using triangle inequality, we have $\dest(x, s_j) \le d(x, s_j) + 2\OPT \le 4\OPT$

\end{proof}



Note that \cref{claim:warmup-med-trick} is sufficient to establish the correctness of the algorithm as the point chosen according to farthest traversal will have distance larger than $4\OPT$. Now that we have a bound on distances, we are ready to prove the approximation guarantee of our algorithm.


% \chen{What is even the definition of $\dtilde(x, \widetilde{C}_j)$ (from the perspective of a reader)?}

%For each $x$, let estimate of distance of point $x$ to the center $s_j$ be \dest$(x,s_j) = \dtilde(x, \widetilde{C}_j)$ for all $j$. 

%We make the following two observations 

% \begin{itemize}
%     \item If $x$ belongs to the ground truth cluster $\Cstar_j$, $d(x, s_j) \le 2\OPT$ and $\dest(x,s_j) \in [0, 4\OPT]$.
%     \item Otherwise, from assumption we have $d(x,s_j) = \omega(1).\OPT$ which gives us
%     \[ \big( 1-o(1) \big)  d(x, s_j) \le \dest(x, s_j) \le \big( 1+o(1) \big) d(x, s_j)\]
% \end{itemize}




%If we use these noisy estimates for furthest traversal, the above two observations are sufficient to establish the correctness as the distance estimate chosen will always be more then 4\OPT. Also, note that the second observation gives us $d(x, s_j) \ge \big( 1-o(1) \big) \dest(x, s_j)$.


\begin{proof}[Proof of \cref{thm:warmup-alg}]
    

To establish the approximation guarantee, assume that at stage $i$, under truthful distance queries, the furthest point is $q^* \in X \setminus T \cup S_{i-1}$ and the corresponding center is $s_u^* \in S_{i-1}$ while under noisy queries the furthest point is $q \in X \setminus T \cup S_{i-1}$ and corresponding center is $s_u \in S_{i-1}$. \chen{We definitely need to explain here.} We have, $d(q^*, s_u^*) \geq d(q, s_u)$ and $\dest(q^*, s_u^*) \leq \dest (q, s_u)$. From \cref{claim:warmup-med-trick},




\begin{align*}
    d(q, s_u)   &\ge \big( 1-o(1) \big) \dest(q, s_u) \\
                &\ge \big( 1-o(1) \big) \dest(q^*, s_u^*) \\
                &\ge \big( 1-o(1) \big)^2 d(q^*, s_u^*) \\
    % \dest(q, s_u) &\ge \big( 1+o(1) \big) \big( 1-o(1) \big)^2 d(q^*, s_u^*) \\
    %             &\ge \big( 1-o(1) \big)^2 d(q^*, s_u^*)
\end{align*} 



To bound the distance of any two points in the set of cluster centers $S_k = \{s_1, \dots ,s_k\}$ returned by the algorithm, for any prefix $S_j = \{s_1, \dots, s_j\}$, let the true farthest point be $q^*_j$ from $S_j$ and let the coverage radius be $d(q^*_k, S_k) = r$. For $i < j \le k$,

\begin{align*}
    d(s_i, s_j) &\geq d(s_j, S_j) \\
                &\geq \big(1 - o(1) \big)^2 d(q^*_j, S_j) \\
                &\geq \big(1 - o(1) \big)^2 d(q^*_k, S_k) \\
                &\geq \big(1 - o(1) \big)^2 r
\end{align*}


The coverage radius of the optimal clustering is $\OPT$. If any two points in $S_k$ belong to the same cluster in optimal clustering, then $\big(1 - o(1) \big)^2 r \leq 2\OPT$ which implies $r = O(1) \OPT$. If all points in $S_k$ belong to different clusters under the optimal clustering, then if $S^*_k$ denotes the optimal cluster centers then for $j \in \{1, \dots, k\}$

$r = \max_{x \in X} d(x, S_k) \leq d(x, S^*_k) + d(s_j, S^*_k) \leq 2\OPT \leq  \frac{2}{\big(1 - o(1) \big)^2}  \OPT$

\end{proof}

% Thus, using the noisy distance estimates we obtain the following guarantee for the furthest distance 

% \[
% ( 1-o(1) )^2 d(q^*, s_u^*) \le \dest(q, s_u) \le ( 1+o(1) )^2 d(q^*, s_u^*)
% \]

% \[c_l B \leq A \leq c_u C\]

% Define $A$
% $ $

% \prat{I think this doesn't care if $s_u = s_u^*$}

%\paragraph{Wrapping up the proof \Cref{thm:warmup-alg}.} Using \Cref{lem:warmup-sample-size} ...






\begin{remark}
To remove the first assumption, we need to manipulate triangle inequality. For the second assumption, we can try non-uniform sampling. 
\end{remark}
